Node-Based Learning of Multiple Gaussian Graphical Models

We consider the problem of estimating high-dimensional Gaussian graphical models corresponding to a single set of variables under several distinct conditions. This problem is motivated by the task of recovering transcriptional regulatory networks on the basis of gene expression data {containing heterogeneous samples, such as different disease states, multiple species, or different developmental stages}. We assume that most aspects of the conditional dependence networks are shared, but that there are some structured differences between them. Rather than assuming that similarities and differences between networks are driven by individual edges, we take a node-based approach, which in many cases provides a more intuitive interpretation of the network differences. We consider estimation under two distinct assumptions: (1) differences between the K networks are due to individual nodes that are perturbed across conditions, or (2) similarities among the K networks are due to the presence of common hub nodes that are shared across all K networks. Using a row-column overlap norm penalty function, we formulate two convex optimization problems that correspond to these two assumptions. We solve these problems using an alternating direction method of multipliers algorithm, and we derive a set of necessary and sufficient conditions that allows us to decompose the problem into independent subproblems so that our algorithm can be scaled to high-dimensional settings. Our proposal is illustrated on synthetic data, a webpage data set, and a brain cancer gene expression data set.

==> figures/png2eps <==
#! /bin/bash
# converts png to eps
#
# 2003-04-09 Thomas Henlich
#
# requires: pngcheck pngtopnm sed basename
#           pnmtotiff tiff2ps
#           bc (for images with non-square pixels)
#
# Usage:
# png2eps file.png > file.eps

# for maximum compression set this to -lzw
# (requires LZW compression in pnmtotiff and tiff2ps)
COMPRESS=-packbits
#COMPRESS=-lzw

# we need a tmp file for input to tiff2ps
OUTFILE=/tmp/png2eps.tif.$$

# temp file for the tEXt chunk
TXTFILE=/tmp/png2eps.txt.$$

# command to remove files
RM="rm -f"

# get the resolution (if specified) from the PNG file
CHK=`pngcheck -v $1`

# get height in pixels from the PNG file
HEIGHT=`echo $CHK | sed -ne 's/.* [0-9]\+ x \(.*\) image.*/\1/p;'`

# a rowsperstrip parameter of 'height' (or more) is needed to generate one 
# single strip of data in the TIFF file (reduces file size)
ROWSPERSTRIP="-rowsperstrip $HEIGHT"
# ROWSPERSTRIP="rowsperstrip 1000000"

# for images with square pixels, pngcheck outputs a line like
#   chunk pHYs ... 9646x9646 pixels/meter (245 dpi)
# and we can read the resolution in dpi directly
RES=`echo $CHK | sed -ne '/pHYs/s/.*(\(.*\) dpi.*/\1/p;'`

# for images with non-square pixels, pngcheck outputs a line like
#   chunk pHYs ... 9646x4803 pixels/meter
XRES=`echo $CHK | sed -ne '/pHYs/s/.*: \([0-9]*\)x.* pixels\/meter.*/\1/p;'`
YRES=`echo $CHK | sed -ne '/pHYs/s/.*x\([0-9]*\) pixels\/meter.*/\1/p;'`

# for images with no fixed resolution, pngcheck may output a line like
#   chunk pHYs ... 9646x4803 pixels/unit
# we ignore it (like pdfTeX does)

# set the command-line arguments for pnmtotiff which specify the resolution
if [ "$RES" ] ; then
  echo "png2eps: Image with square pixels ($RES dpi)" 1>&2
  RES='-xres '$RES' -yres '$RES
fi
if [ -z "$RES" ] ; then
  if [ "$XRES" ] ; then
    echo "png2eps: Image with non-square pixels" \
      "($XRES""x$YRES pixels/meter)" 1>&2
# we still have to convert pixels/meter -> dpi
    RES='-xres '`echo .0254*$XRES |bc`' -yres '`echo .0254*$YRES |bc`;
  else
# no resolution was specified and so a default of 72 dpi will be used
    echo "png2eps: No resolution specified, using default (72 dpi)" 1>&2;
  fi
fi

# convert to tiff
pngtopnm -verbose -text $TXTFILE $1 | \
pnmtotiff $ROWSPERSTRIP $RES $COMPRESS -indexbits=1,2,4,8 >$OUTFILE

# get the title of the figure
TITLE="`sed -ne 's/^Title *\(.*\)/\1/p;' <$TXTFILE`"
# set to input file name if unspecified
[ -z "$TITLE" ] && TITLE=`basename $1`

# convert to EPS, replacing the %%Title comment
tiff2ps -2 -e -z $OUTFILE | sed -e "s/^\(%%Title: \).*/\1$TITLE/;"

# remove temp files
$RM $OUTFILE $TXTFILE

